Learning the Graphical Structure of Electronic Health Records with Graph Convolutional Transformer

Effective modeling of electronic health records (EHR) is rapidly becoming an important topic in both academia and industry. A recent study showed that using the graphical structure underlying EHR data (e.g. relationship between diagnoses and treatments) improves the performance of prediction tasks such as heart failure prediction. However, EHR data do not always contain complete structure information. Moreover, when it comes to claims data, structure information is completely unavailable to begin with. Under such circumstances, can we still do better than just treating EHR data as a flat-structured bag-of-features? In this paper, we study the possibility of jointly learning the hidden structure of EHR while performing supervised prediction tasks on EHR data. Specifically, we discuss that Transformer is a suitable basis model to learn the hidden EHR structure, and propose Graph Convolutional Transformer, which uses data statistics to guide the structure learning process. The proposed model consistently outperformed previous approaches empirically, on both synthetic data and publicly available EHR data, for various prediction tasks such as graph reconstruction and readmission prediction, indicating that it can serve as an effective general-purpose representation learning algorithm for EHR data.

==> attention.tex <==
\subsection{Attention Behavior}
\label{ssec:exp_attention}
\begin{figure}[h]
\centering
\includegraphics[width=.48\textwidth]{figs/attention_hypertension}
\caption{Attention by hypertension.}
\label{fig:attention_hypertension}
\end{figure}
\begin{figure}[h]
\centering
\includegraphics[width=.48\textwidth]{figs/attention_warfarin}
\caption{Attention by warfarin.}
\label{fig:attention_fwarfarin}
\end{figure}
The previous section showed that Transformer outperformed various baseline approaches in all \numtasks tasks, and the proposed variant, \mname, showed further improvement. In this section, we show the attention of \mname to qualitatively demonstrate that \mname learns different patterns for different features.
\note{dusenberrymw: Given space constraints, there may not be enough room to give attention an adequate treatment. If that ends up being the case, I don't think it would detract from the paper to add it to the appendix and then include in the full paper.}

==> experiments_old.tex <==
\subsection{Synthetic Encounter Record}
\label{ssec:exp_synthetic}
\cite{choi2018mime} evaluated their model on proprietary EHR data that contained structure information.
Unfortunately, to the best of our knowledge, there are no publicly available EHR data that contain structure information (which is the main motivation of this work).
In order to evaluate \mname's ability to learn EHR structure, we instead generated synthetic data that has a similar structure as EHR data.

The synthetic data has the same \textit{visit-diagnosis-treatment-lab results} hierarchy as EHR data, and was generated in a top-down fashion.
Each level was generated conditioned on the previous level, where the probabilities were modeled with the Pareto distribution.
Pareto distribution follows the power law which best captures the long-tailed nature of medical codes.
Using 1000 diagnosis codes, 1000 treatment codes, and 1000 lab codes, we initialized $p(D), p(D|D), p(M|D), p(R|M,D)$ to follow the Pareto distribution, where $D, M$, and $R$ respectively denote diagnosis, treatment, and lab random variables.
$p(D)$ is used to draw independent diagnosis codes $d_i$, and $p(D|D)$ is used to draw $d_j$ that are likely to co-occur with the previously sampled $d_i$.
$P(M|D)$ is used to draw a treatment code $m_j$, given some $d_i$.
$P(R|M,D)$ is used to draw a lab code $r_k$, given some $m_j$ and $d_i$.
Detailed description of generating the synthetic records and the link to download them are provided in Appendix~\ref{appendix:synthetic}, and Appendix~\ref{appendix:data_share}, respectively.
Code for generating the synthetic records will be open-sourced in the future.
Table~\ref{table:data_stat} summarizes the data statistics.

\subsection{eICU Collaborative Research Dataset}
\label{ssec:exp_eicu}
\input{tables/data_stats.tex}
To test \mname on real-world EHR records, we use Philips eICU Collaborative Research Dataset\footnote{https://eicu-crd.mit.edu/about/eicu/} \cite{pollard2018eicu}.
eICU consists of Intensive Care Unit (ICU) records filtered for remote caregivers, collected from multiple sites in the United States between 2014 and 2015.
From the encounter records, medication orders and procedure orders, we extracted diagnosis codes and treatment codes (\textit{i.e.} medication, procedure codes).
Since the data were collected from an ICU, a single encounter can last several days, where the encounter structure evolves over time, rather than being fixed as Figure~\ref{fig:ehr_graph}.
Therefore we used encounters where the patient was admitted for less than 24 hours, and removed duplicate codes (\textit{i.e.} medications administered multiple times).
Additionally, we did not use lab results as their values change over time in the ICU setting (\textit{i.e.} blood pH level).
We leave as future work how to handle ICU records that evolve over a longer period of time.
Note that eICU does not contain structure information.
For example, we know that \textit{cough} and \textit{acetaminophen} in Figure~\ref{fig:ehr_graph} occur in the same visit, but do not know if \textit{acetaminophen} was prescribed due to \textit{cough}.
Table~\ref{table:data_stat} summarizes the data statistics.

\input{tables/recon_dt_aucpr.tex}
\subsection{Baseline Models}
\label{ssec:exp_baselines}
\begin{itemize}[leftmargin=5.5mm]
\item \textbf{GCN}: Given the true adjacency matrix $\Ab$, we follow Eq.~\eqref{eq:gin} to learn the feature representations $\cb_i$ of each feature $c_i$ in a visit $\mathcal{V}$.
The visit embedding $\vb$ (\textit{i.e.} graph-level representation) is obtained from the placeholder visit node $v$.
This model will serve as the optimal model during the experiments.
\item \textbf{GCN$_{P}$}: Instead of the true adjacency matrix $\Ab$, we use the conditional probability matrix $\Pb$, and follow Eq.~\eqref{eq:gin}.
\item \textbf{GCN$_{random}$}: Instead of the true adjacency matrix $\Ab$, we use a randomly generated normalized adjacency matrix where each element is indepdently sampled from a uniform distribution between 0 and 1.
This model will let us evaluate whether true encounter structure is useful at all.
\item \textbf{Shallow}: Each $c_i$ is converted to a latent representation $\cb_i$ using multi-layer feedforward networks with ReLU activations.
The visit representation $\vb$ is obtained by simply summing all $\cb_i$'s.
We use layer normalization \cite{ba2016layer}, drop-out \cite{srivastava2014dropout} and residual connections \cite{he2016deep} between layers.
%This is equivalent to taking the node embeddings $\cb_i$'s (\textit{i.e.} columns of $\Wb_x$) in the visit $\mathcal{V}$, and summing them up to derive a single vector $\vb$.
%\item \textbf{non-linear}: The binary vector $\xb$ is transformed to a visit embedding $\vb = \sigma(\Wb_x \xb)$ where we use \textit{ReLU} for $\sigma(\cdot)$ to add non-linearity to \textbf{linear}.
\item \textbf{Deep}: We use multiple feedforward layers with ReLU activations (including layer normalization, drop-out and residual connections) on top of \textbf{shallow} to increase the expressivity.
Note that \cite{zaheer2017deep} theoretically describes that this model is sufficient to obtain the optimal representation of a set of items (\textit{i.e.,} a visit consisting of multiple features).
\end{itemize}

\subsection{Prediction Tasks}
\label{ssec:exp_task}
In order to evaluate the model's capacity to leverage the implicit encounter structure, we use prediction tasks based on a single encounter, rather than a sequence of encounters, which was the experiment setup in \cite{choi2018mime}.
Specifically, we test the models on the following tasks.
Parentheses indicate which dataset is used for each task.
\begin{itemize}[leftmargin=5.5mm]
\item \textbf{Graph reconstruction (Synthetic)}: Given an encounter with $N$ features, we train models to learn $N$ feature embeddings $\Cb$, and predict whether there is an edge between every pair of features, by performing an inner-product between each feature embedding pairs $\cb_i$ and $\cb_j$ (\textit{i.e.} $N^2$ binary predictions).
We do not use \textbf{Deep} baseline for this task, as we need individual embeddings for all features $c_i$'s.
\item \textbf{Diagnosis-Treatment classification (Synthetic)}: We assign labels to an encounter if there are specific diagnosis ($d_1$ and $d_2$) and treatment code ($m_1$) connections.
Specifically, we assign label "1" if the encounter contains $d_1$-$m_1$ connection, and label "2" if the encounter contains $d_2$-$m_1$ connection.
We intentionally made the task difficult so that the models cannot achieve a perfect score by just basing their prediction on whether $d_1$, $d_2$ and $m_1$ exist in an encounter.
The prevalence for both labels are approximately $3.3\%$.
Further details on the labels are provided in Appendix~\ref{appendix:dxtreatment}. This is a multi-label prediction task using the visit representation $\vb$.
%Further detail on the conditional probabilities of \textit{Diagnosis1}, \textit{Diagnosis2} and \textit{Treatment1} are provided in Appendix~\ref{appendix:dxtreatment}.
\item \textbf{Masked diagnosis code prediction (Synthetic, eICU)}: Given an encounter record, we mask a random diagnosis code $d_i$. We train models to learn the embedding of the masked code to predict its identity, \textit{i.e.} a multi-class prediction. For \textbf{Shallow} and \textbf{Deep}, we use the visit embedding $\vb$ as a proxy for the masked code representation.
The row and the column of the conditional probability matrix $\Pb$ that correspond to the masked diagnosis were also masked to zeroes.
\item \textbf{Readmission prediction (eICU)}: Given an encounter record, we train models to learn the visit embedding $\vb$ to predict whether the patient will be admitted to the ICU again during the same hospital stay, \textit{i.e.,} a binary prediction. The prevalence is approximately $17.2\%$.
\item \textbf{Mortality prediction (eICU)}: Given an encounter record, we train models to learn the visit embedding $\vb$ to predict patient death during the ICU admission, \textit{i.e.,} a binary prediction. The prevalence is approximately $7.3\%$.
%\item \textbf{Medications prediction}: Given an encounter record with all medication codes removed, we train models to learn the visit representation $\vb$ to predict all medication codes, \textit{i.e.,} a multi-label prediction with the output dimension the size of the medication vocabulary.
%\item \textbf{Future diagnosis prediction}: Given an outpatient encounter, we train models to learn $\vb$ to predict all diagnosis codes of the next encounter \textit{i.e.} a multi-label prediction with the output dimension the size of the diagnosis vocabulary.
\end{itemize}
For each task, data were randomly divided into train, validation, and test set in 8:1:1 ratio for 5 times, yielding 5 trained models, and we report the average performance.
Note that the conditional probability matrix $\Pb$ was calculated only with the training set.
Further training details and hyperparameter settings are described in Appendix~\ref{appendix:implementation}.

\subsection{Prediction Performance}
\label{ssec:exp_result}
%\input{tables/graph_recon_dt_pred_result.tex}
%\input{tables/graph_recon_dt_pred_result2.tex}
%\input{tables/graph_recon_result.tex}
%f\input{tables/dt_pred_result.tex}
\input{tables/node_pred_result2.tex}
%\input{tables/mortality_readmission_result.tex}
%\input{tables/readmission_mortality_result.tex}
\input{tables/readmission_mortality_aucpr.tex}
%\input{tables/rx_pred_result.tex}
%\input{tables/dx_pred_result.tex}
Table~\ref{table:graph_recon_dt_pred_result} shows the graph reconstruction performance and the diagnosis-treatment classification performance of all models.
Naturally, GCN shows the best performance since it uses the true adajcency matrix $\Ab$. 
Given that GCN$_P$ is outperformed only by \mname, we can infer that the conditional probability is indeed indicative of the true structure.
\mname, which combines the strength of both GCN$_P$ and Transformer shows the best performance, besides GCN.
It is noteworthy that GCN$_{random}$ outperforms Shallow.
This seems to indicate that for graph reconstruction, attending to other features, regardless of how accurately the process follows the true structure, is better than individually embedding each feature.
Diagnosis-treatment classification, on the other hand, clearly penalizes randomly attending to the features, since GCN$_{random}$ shows the worst performance.
\mname again shows the best performance.

Table~\ref{table:node_pred_result} shows the model performance for masked diagnosis prediction for both datasets.
GCN could not be evaluated on eICU, since eICU does not have the true structure.
However, GCN naturally shows the best performance on the synthetic dataset.
%GCN$_{random}$ again demonstrates performance for both datasets, indicating that inferring a diagnosis based on other features requires accurate structure knowledge.
Interestingly, Transformer shows comparable performance to GCN$_{random}$, indicating the opposite nature of this task compared to graph reconstruction, where simply each feature attending to other features significantly improved performance.
Note that the task performance is significantly higher for eICU than for the synthetic dataset.
This is mainly due to eICU having a very skewed diagnosis code distribution.
In eICU, more than 80\% of encounters have diagnosis codes related to whether the patient has been in an operating room prior to the ICU admission. 
Therefore randomly masking one of them does not make the prediction task as difficult as for the synthetic dataset.
%Interestingly, both GCN$_P$ and \mname show strong performance on both datasets, but the performance gap is significantly wider for eICU.
%fThis seems due to the fact that eICU has a larger diagnosis code vocabulary than the synthetic dataset (2460 vs 1000), which makes guessing the correct diagnosis code harder.
%Also, eICU data volume is smaller than the synthetic dataset (33168 vs 50000), making the already harder task even more difficult for other models.
%Both GCN$_P$ and \mname, however, relies on the prior knowledge extracted from the training set, which is a form of rather strong regularization, making both models robust to the smaller dataset.

Table~\ref{table:mortality_readmission_result} shows the readmission prediction and mortality prediction performance of all models on eICU.
As shown by \mname's superior performance, it is evident that readmission prediction benefits from using the latent encounter structure.
Mortality prediction, on the other hand, seems to rely little on the encounter structure, as can be seen from the marginally superior performance of \mname compared to Transformer and Deep.
%demonstrate strikingly contrasting performance indicates that mortality prediction on eICU data relies little to the true structure.
%Rather, given the comparable performances of Shallow, it seems that mortality prediction can be successfully performed by simply adding all features.
%This seems natural, since eICU records are filtered for remote caregivers, who do not necessarily need to know information indicating patient death.
Even when the encounter structure seems unnecessary, however, \mname still outperforms all other models, demonstrating its potential to be used as a general-purpose EHR modeling algorithm.
%and it should be acting as a regularized Transformer, rather than trying to recover the true structure.
These two experiments indicate that not all prediction tasks require the true encounter structure, and it is our future work to apply \mname to various prediction tasks to evaluate its effectiveness.

%, Table~\ref{table:node_pred_result}, and Table~\ref{table:mortality_pred_result} respectively show mortality prediction performance, medication prediction performance, and masked diagnosis code prediction performance for all models on two datasets.

%fIn both mortality prediction and medication prediction, all models show stronger performance on MIMIC-III than eICU, which is reasonable given that MIMIC-III's encounter records are more dense, \textit{i.e.} there are more features per encounter on average as shown by Table~\ref{table:data_stat}.
%fIn masked code prediction, on the other hand, all models show stronger performance on eICU, naturally because eICU's diagnosis code vocabulary is smaller.
%fFurthermore, as MIMIC-III's encounter has more diagnosis codes on average, it is more likely for the models to predict one of the visible diagnosis codes.

%fAs all three tables show, Transformer outperforms baseline models on all \numtasks tasks on two different datasets.
%fThis empirical evidence strongly indicates Transformer's suitability to be used as a general-purpose EHR encounter modeling framework.
%fFinally, Transformer significantly outperforms baseline models on some tasks and datasets, while the perforamnce improvement is not as dramatic for other tasks and datasets, which requires further investigation in the future.
%fWe discuss Transformer's attention behavior in Appendix~\ref{appendix:attention}.

\subsection{Evaluating the Learned Encounter Structure}
\label{ssec:encounter_structure}
%Even though the ultimate goal of \mname is to outperform the \textit{bag-of-features} approach in prediction tasks on encounter records, the premise was that \mname is able to achieve this by effectively learning the encounter structure, even when the structure information is unavailable.
In this section, we analyze the learned structure of both Transformer and \mname.
As we know the true structure $\Ab$ of synthetic records, we can evaluate how well both models learned $\Ab$ via self-attention $\hat{\Ab}$.
Since we can view the normalized true adjacency matrix $\tilde{\Db}^{-1} \tilde{\Ab}$ as a probability distribution, we can measure how well the attention map $\hat{\Ab}$ in Eq.~\eqref{eq:define_adj} approximates $\tilde{\Db}^{-1} \tilde{\Ab}$ using KL divergence $D_{KL}(\tilde{\Db}^{-1} \tilde{\Ab} || \hat{\Ab})$.
%\input{tables/structure_eval.tex}
\input{tables/structure_eval2.tex}
Table~\ref{table:structure_eval} shows the KL divergence between the normalized true adjacency and the learned attention on the test set of the synthetic data while performing three different tasks.
For GCN$_P$, the adjacency matrix is fixed to the conditional probability matrix $\Pb$, so KL divergence can be readily calculated. 
For Transformer and \mname, we calculated KL divergence between $\tilde{\Db}^{-1} \tilde{\Ab}$ and the attention maps in each self-attention block, and averaged the results.
We repeated this process for 5 times (on 5 randomly sampled train, validation, test sets) and report the average performance.
Note that KL divergence can be lowered by evenly distributing the attention across all features, which is the opposite of learning the encounter structure.
Therefore we also show the entropy of $\hat{\Ab}$ alongside the KL divergence.

As shown by Table~\ref{table:structure_eval}, the conditional probabilities are closer to the true structure than what Transformer has learned, in all three tasks.
\mname shows similar performance to GCN$_P$ in all tasks, and was even able to improve upon $\Pb$ in both graph reconstruction and diagnosis-treatment classification tasks.
%Interestingly, it seems graph reconstruction can be done quite well even if the model deviates much from the true structure. Transformer's attention was significantly dissimilar to the true structure compared to GCN$_P$, but it was still able to outperform GCN$_P$.
It is notable that, despite having attentions significantly different from the true structure, Transformer demonstrated strong graph reconstruction performance in Table~\ref{table:graph_recon_dt_pred_result}.
This again indicates the importance of simply attending to other features in graph reconstruction, which was discussed in Section~\ref{ssec:exp_result} regarding the performance of GCN$_{random}$.
For the other two tasks, regularizing the models to stay close to $\Pb$ helped \mname outperform Transformer as well as other models.
%This seems to be due to the fact that graph reconstruction requires the features to ``see'' one another at least once to determine
We show visual examples of attention behavior of both Transformer and \mname in Appendix~\ref{appendix:attention}.

==> tables/dt_pred_result.tex <==
\begin{table}[h]
\caption{Diagnosis-Treatment classification performance}
\label{table:dt_pred_result}
\footnotesize
%\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{lcccc}
\hline
Model & \begin{tabular}{@{}c@{}} Validation\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUORC\end{tabular}\\
\hline
GCN & 1.0 & 1.0 & 1.0 & 1.0 \\
GCN$_P$ & 0.9164 & 0.9934 & 0.9175 & 0.9931\\
Shallow & 0.9235 & 0.9935 & 0.9103 & 0.9926\\
Deep & 0.9173 & 0.9936 & 0.9070 & 0.9923\\
Transformer & 0.9293 & 0.9942 & 0.9146 & 0.9930\\
\mname & 0.9270 &0.9942 & 0.9201 & 0.9933\\
\hline
\end{tabular}
%f}
\end{table}

==> tables/dx_pred_result.tex <==
\begin{table}[h]
\caption{Future diagnosis prediction performance}
\label{table:dx_pred_result}
\small
\centering
\begin{tabular}{lcccc}
\hline
 & Loss & AUC-PR & Recall@5 & Recall@10\\
\hline
raw & 0 & 0 & 0 & 0\\
linear & 0 & 0 & 0 & 0\\
non-linear & 0 & 0 & 0 & 0\\
MLP & 0 & 0 & 0 & 0\\
Transformer & 0 & 0 & 0 & 0\\
GCT & 0 & 0 & 0 & 0\\
\hline
\end{tabular}
\end{table}

==> tables/graph_recon_dt_pred_result.tex <==
\begin{table}[t]
\caption{Graph reconstruction and diagnosis-treatment classification performance.}
\vspace{1mm}
\label{table:graph_recon_dt_pred_result}
\footnotesize
\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{lcccccccc}
% \hline
\toprule
& \multicolumn{4}{c}{\textbf{Graph reconstruction}} & \multicolumn{4}{c}{\textbf{Diagnosis-Treatment classification}}\\
%\hline
Model & \begin{tabular}{@{}c@{}} Validation\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUROC\end{tabular}\\
% \hline
\midrule
GCN & 0.9999 & 1.0 & 0.9999 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\
% \hline
\midrule
GCN$_P$ & 0.5863 & 0.8894 & 0.5826 & 0.8887 & 0.9164 & 0.9934 & 0.9175 & 0.9931\\
GCN$_{random}$ & 0.5657 & 0.8807 & 0.5614 & 0.8803 & 0.8973 & 0.9916 & 0.8900 & 0.9903\\
Shallow & 0.5482 & 0.8589 & 0.5444 & 0.8582 & 0.9235 & 0.9935 & 0.9103 & 0.9926\\
Deep & - & - & - & - & 0.9173 & 0.9936 & 0.9070 & 0.9923\\
Transformer & 0.5944 & 0.8925 & 0.5885 & 0.8910 & \textbf{0.9293} & \textbf{0.9942} & 0.9146 & 0.9930\\
\mname & \textbf{0.6063} & \textbf{0.8966} & \textbf{0.6003} & \textbf{0.8956} & 0.9291 & \textbf{0.9942} & \textbf{0.9219} & \textbf{0.9933}\\
% \hline
\bottomrule
\end{tabular}
}
\end{table}

==> tables/graph_recon_dt_pred_result2.tex <==
\begin{table}[t]
\caption{Graph reconstruction and diagnosis-treatment classification performance. Parentheses denote standard deviation.}
\vspace{1mm}
\label{table:graph_recon_dt_pred_result}
\footnotesize
\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{lcccccccc}
% \hline
\toprule
& \multicolumn{4}{c}{\textbf{Graph reconstruction}} & \multicolumn{4}{c}{\textbf{Diagnosis-Treatment classification}}\\
%\hline
Model & \begin{tabular}{@{}c@{}} Validation\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUROC\end{tabular}\\
% \hline
\midrule
GCN & 100 (0.0) & 100 (0.0) & 100 (0.0) & 100 (0.0) & 100 (0.0) & 100 (0.0) & 100 (0.0) & 100 (0.0)\\
% \hline
\midrule
GCN$_P$ & 58.07 (0.19) & 88.70  (0.11) & 58.00 (0.21)  & 88.65 (0.05) & 84.39 (1.66) & 94.93 (1.27) & 84.43 (2.14) & 94.75 (1.35)\\
GCN$_{random}$ & 56.44 (0.18) & 88.06 (0.09) & 56.35 (0.21) & 87.99 (0.08) & 78.39 (1.44) & 92.30 (0.53) & 78.04 (2.14) & 92.21 (0.70)\\
Shallow & 54.43 (0.15) & 85.78 (0.10) & 54.41 (0.17) & 85.73 (0.05) & 85.30 (1.81) & 95.75 (1.16) & 85.55 (2.06) & 95.84 (1.40)\\
Deep & - & - & - & - & 82.10 (0.96) & 93.87 (0.71) & 81.98 (0.46) & 93.74 (0.41)\\
Transformer & 57.55 (0.20) & 88.43 (0.13) & 57.52 (0.15) & 88.44 (0.08) & 83.29 (2.82) & 94.94 (2.26) & 83.80 (1.78) & 94.93 (2.10)\\
\mname & \textbf{59.72} (0.27) & \textbf{89.36} (0.12) & \textbf{59.65} (0.31) & \textbf{89.31} (0.13) & \textbf{86.86} (1.03) & \textbf{96.26} (1.46) & \textbf{86.71} (2.47) & \textbf{96.00} (1.54)\\
% \hline
\bottomrule
\end{tabular}
}
\end{table}

==> tables/graph_recon_result.tex <==
\begin{table}[h]
\caption{Graph reconstruction performance}
\label{table:graph_recon_result}
\footnotesize
%\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{lcccc}
\hline
Model & \begin{tabular}{@{}c@{}} Validation\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUORC\end{tabular}\\
\hline
GCN & 0.9999 & 1.0 & 0.9999 & 1.0 \\
GCN$_P$ & 0.5503 & 0.8595 & 0.5461 & 0.8587\\
Shallow & 0.5482 & 0.8589 & 0.5444 & 0.8582\\
Transformer & 0.5944 & 0.8925 & 0.5885 & 0.8910\\
\mname & 0.6063 & 0.8966 & 0.6003 & 0.8956\\
\hline
\end{tabular}
%f}
\end{table}

==> tables/hyper_graph_recon.tex <==
\begin{table}[h]
\caption{Hyperparameters for graph reconstruction on the synthetic data.}
\vspace{1mm}
\label{table:hyper_graph_recon}
\footnotesize
\centering
\begin{tabular}{lcccccc}
% \hline
\toprule
& GCN & GCN$_P$ & GCN$_{random}$ & Shallow & Transformer & \mname\\
% \hline
\midrule
Learning rate & 0.00045 & 0.0006 & 0.0003 & 0.00025 & 0.0007 & 0.0005\\
MLP dropout rate & 0.3 & 0.01 & 0.5 & 0.2 & 0.8 & 0.3\\
Post-MLP dropout rate & 0.2 & 0.02 & 0.005 & - & 0.001 & 0.1\\
Regularization coef. & - & - & - & - & - & 0.02\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\caption{Hyperparameters for diagnosis-treatment classification on the synthetic data.}
\vspace{1mm}
\label{table:hyper_dt_classification}
\footnotesize
\centering
\begin{tabular}{lccccccc}
% \hline
\toprule
& GCN & GCN$_P$ & GCN$_{random}$ & Shallow & Deep & Transformer & \mname\\
% \hline
\midrule
Learning rate & 0.0001 & 0.0001 & 0.0001 & 0.0002 & 0.0008 & 0.00015 & 0.0001\\
MLP dropout rate & 0.2 & 0.3 & 0.5 & 0.02 & 0.01 & 0.5 & 0.85\\
Post-MLP dropout rate & 0.65 & 0.02 & 0.4 & - & 0.3 & 0.01 & 0.03\\
Regularization coef. & - & - & - & - & - & - & 0.05\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\caption{Hyperparameters for masked diagnosis code prediction on the synthetic data.}
\vspace{1mm}
\label{table:hyper_node_pred_synthetic}
\footnotesize
\centering
\begin{tabular}{lccccccc}
% \hline
\toprule
& GCN & GCN$_P$ & GCN$_{random}$ & Shallow & Deep & Transformer & \mname\\
% \hline
\midrule
Learning rate & 0.0003 & 0.0007 & 0.0002 & 0.0007 & 0.0004 & 0.0003 & 0.0001\\
MLP dropout rate & 0.01 & 0.8 & 0.5 & 0.08 & 0.12 & 0.4 & 0.85\\
Post-MLP dropout rate & 0.88 & 0.005 & 0.5 & - & 0.75 & 0.5 & 0.6\\
Regularization coef. & - & - & - & - & - & - & 0.05\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\caption{Hyperparameters for masked diagnosis code prediction on eICU.}
\vspace{1mm}
\label{table:hyper_node_pred_eicu}
\footnotesize
\centering
\begin{tabular}{lcccccc}
% \hline
\toprule
& GCN$_P$ & GCN$_{random}$ & Shallow & Deep & Transformer & \mname\\
% \hline
\midrule
Learning rate & 0.0005 & 0.0001 & 0.0001 & 0.00012 & 0.0001 & 0.0009\\
MLP dropout rate & 0.5 & 0.3 & 0.3 & 0.4 & 0.87 & 0.5\\
Post-MLP dropout rate & 0.5 & 0.4 & - & 0.45 & 0.2 & 0.03\\
Regularization coef. & - & - & - & - & - & 50.0\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\caption{Hyperparameters for readmission prediction on eICU.}
\vspace{1mm}
\label{table:hyper_readmission}
\footnotesize
\centering
\begin{tabular}{lcccccc}
% \hline
\toprule
& GCN$_P$ & GCN$_{random}$ & Shallow & Deep & Transformer & \mname\\
% \hline
\midrule
Learning rate & 0.00024 & 0.0001 & 0.0001 & 0.00011 & 0.0002 & 0.00022\\
MLP dropout rate & 0.3 & 0.7 & 0.63 & 0.05 & 0.45 & 0.08\\
Post-MLP dropout rate & 0.1 & 0.01 & - & 0.33 & 0.28 & 0.024\\
Regularization coef. & - & - & - & - & - & 0.1\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\caption{Hyperparameters for mortality prediction on eICU.}
\vspace{1mm}
\label{table:hyper_mortality}
\footnotesize
\centering
\begin{tabular}{lcccccc}
% \hline
\toprule
& GCN$_P$ & GCN$_{random}$ & Shallow & Deep & Transformer & \mname\\
% \hline
\midrule
Learning rate & 0.0003 & 0.00013 & 0.0001 & 0.00015 & 0.0006 & 0.00011\\
MLP dropout rate & 0.85 & 0.9 & 0.25 & 0.01 & 0.88 & 0.72\\
Post-MLP dropout rate & 0.04 & 0.01 & - & 0.01 & 0.2 & 0.005\\
Regularization coef. & - & - & - & - & - & 1.5\\
\bottomrule
\end{tabular}
\end{table}

==> tables/mortality_pred_result.tex <==
\begin{table}[t]
\caption{Mortality prediction performance on eICU.}
\vspace{1mm}
\label{table:mortality_pred_result}
\footnotesize
%\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{lcccc}
% \hline
\toprule
Model & \begin{tabular}{@{}c@{}} Validation\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUROC\end{tabular}\\
% \hline
\midrule
GCN$_P$ & 0.5946 & 0.8746 & 0.6462 & 0.8938\\
GCN$_{random}$ & 0.6312 & 0.8963  & 0.6902 & 0.9138\\
Shallow & 0.6436 & 0.8887 & 0.6783 & 0.9008\\
Deep & 0.6484 & 0.8987 & 0.6903 & 0.9127\\
Transformer & \textbf{0.6666} & 0.9020 & 0.6911 & 0.9110\\
\mname & 0.6530 & \textbf{0.9036} & \textbf{0.6978} & \textbf{0.9184}\\
% \hline
\bottomrule
\end{tabular}
%f}
\end{table}
\vspace{-3mm}

==> tables/mortality_readmission_result.tex <==
\begin{table}[t]
\caption{Readmission prediction and mortality prediction performance on eICU. Parentheses denote standard deviations.}
\vspace{1mm}
\label{table:mortality_readmission_result}
\footnotesize
\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{lcccccccc}
% \hline
\toprule
& \multicolumn{4}{c}{\textbf{Readmission prediction}} & \multicolumn{4}{c}{\textbf{Mortality prediction}}\\
%\hline
Model & \begin{tabular}{@{}c@{}} Validation\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUROC\end{tabular}\\
% \hline
\midrule
GCN$_P$ & 0.4952 & 0.7327 & 0.4706 & \textbf{0.7422} & 0.6664 & 0.9153 & 0.6082 & 0.9066\\
GCN$_{random}$ & 0.4740 & 0.6948 & 0.4421 & 0.6953 & 0.6592 & 0.9196 & 0.5996 & 0.9098\\
Shallow & 0.3962 & 0.6852 & 0.3517 & 0.6740 & 0.6687 & 0.9206 & 0.6120 & 0.9120\\
Deep & 0.4527 & 0.7170 & 0.4429 & 0.7403 & 0.6724 & 0.9213 & 0.6023 & 0.9110\\
Transformer & 0.5057 & 0.7341 & 0.4571 & 0.7161 & 0.6594 & 0.9120 & 0.6039 & 0.9102\\
\mname & \textbf{0.5279} & \textbf{0.7345} & \textbf{0.4837} & 0.7421 & \textbf{0.6757} & \textbf{0.9209} & \textbf{0.6178} & \textbf{0.9122}\\
% \hline
\bottomrule
\end{tabular}
}
\end{table}

==> tables/node_pred_result.tex <==
\begin{table}[t]
\caption{Masked diagnosis code prediction performance on the two datasets.}
\label{table:node_pred_result}
\footnotesize
%\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{lcccc}
% \hline
\toprule
%Dataset & Model & \begin{tabular}{@{}c@{}} Validation\\Accuracy\end{tabular} & \begin{tabular}{@{}c@{}} Test\\Accuracy\end{tabular}\\

& \multicolumn{2}{c}{\textbf{Synthetic}} & \multicolumn{2}{c}{\textbf{eICU}}\\
%\hline
Model & \begin{tabular}{@{}c@{}} Validation\\Accuracy\end{tabular} & \begin{tabular}{@{}c@{}} Test\\Accuracy\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\Accuracy\end{tabular} & \begin{tabular}{@{}c@{}} Test\\Accuracy\end{tabular}\\
% \hline
\midrule
GCN & 0.2828 & 0.3024 & - & -\\
% \hline
\midrule
%GCN$_P$ & 0.1908 & 0.2096 & 0.3271 & 0.3229\\
GCN$_P$ & 0.1908 & 0.2096 & 0.7510 & 0.7389\\
%GCN$_{random}$ & 0.1780 & 0.1980 & 0.2556 & 0.2685\\
GCN$_{random}$ & 0.1780 & 0.1980 & 0.7184 & 0.7137\\
%Shallow & 0.2006 & 0.2156 & 0.2732 & 0.2703\\
Shallow & 0.2006 & 0.2156 & 0.7387 & 0.7241\\
%Deep & 0.1900 & 0.2048 & 0.2785 & 0.2785\\
Deep & 0.1900 & 0.2048 & 0.7406 & 0.7343\\
%Transformer & 0.1962 & 0.2026 & 0.2694 & 0.2703\\
Transformer & 0.1962 & 0.2026 & 0.7295 & 0.7158\\
%\mname & \textbf{0.2182} & \textbf{0.2328} & \textbf{0.3915} & \textbf{0.3929}\\
\mname & \textbf{0.2182} & \textbf{0.2328} & \textbf{0.7796} & \textbf{0.7644}\\
% \hline
\bottomrule
 %& GCN & 0.2828 & 0.3024\\
 %f& GCN$_P$ & 0.1908 & 0.2096\\
 %f& shallow & 0.3488 & 0.3417\\
%feICU & deep & 0.3549 & 0.3547\\
 %f& Transformer & 0.3647 & 0.3581\\
 %f& \mname & 0.2182 & 0.2328\\
%f\hline
\end{tabular}
%f}
\end{table}

==> tables/readmission_mortality_result.tex <==
\begin{table}[t]
\caption{Readmission prediction and mortality prediction performance on eICU.}
\vspace{1mm}
\label{table:mortality_readmission_result}
\footnotesize
\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{lcccccccc}
% \hline
\toprule
& \multicolumn{4}{c}{\textbf{Readmission prediction}} & \multicolumn{4}{c}{\textbf{Mortality prediction}}\\
%\hline
Model & \begin{tabular}{@{}c@{}} Validation\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUROC\end{tabular}\\
% \hline
\midrule
GCN$_P$ & 51.21 (1.54) & 74.03 (0.78) & 49.87 (1.05) & 73.55 (0.81) & 58.08 (3.31) & 89.71 (0.47) & 56.47 (2.01) & 89.53 (0.65)\\
GCN$_{random}$ & 50.78 (1.16) & 72.43 (0.46) & 49.74 (1.73) & 72.59 (0.80) & 57.17 (5.71) & 89.39 (2.43) & 54.35 (6.44) & 89.41 (2.20)\\
Shallow & 37.04 (1.23) & 67.94 (1.29) & 35.09 (1.44) & 67.34 (1.01) & 60.41 (2.53) & 90.00 (0.83) & 57.95 (2.58) & 89.72 (0.38)\\
Deep & 52.19 (1.82) & 74.78 (1.24) & 50.50 (1.26) & 74.12 (0.74) & 57.77 (1.88) & 88.65 (0.93) & 56.05 (1.31) & 89.24 (1.03)\\
Transformer & 51.04 (1.59) & 73.33 (0.65) & 49.99 (1.27) & 73.01 (1.01) & 60.69 (2.91) & 90.89 (1.21) & 59.31 (2.11) & 90.17 (1.52)\\
\mname & \textbf{53.13} (1.24) & \textbf{75.25} (1.28) & \textbf{52.44} (1.42) & \textbf{75.02} (1.14) & \textbf{61.96} (2.59) & \textbf{90.89} (0.52) & \textbf{59.92} (2.23) & \textbf{91.20} (0.48)\\
% \hline
\bottomrule
\end{tabular}
}
\end{table}

==> tables/rx_pred_result.tex <==
\begin{table}[h]
\caption{Medication prediction performance}
\label{table:rx_pred_result}
\footnotesize
\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{clcccc}
\hline
Dataset & Model & \begin{tabular}{@{}c@{}} Validation\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\AUROC\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUCPR\end{tabular} & \begin{tabular}{@{}c@{}} Test\\AUORC\end{tabular}\\
\hline
 & shallow & 0.6318 & 0.9856 & 0.6253 & 0.9856\\
MIMIC-III & deep & 0.6447 & 0.9869 & 0.6402 & 0.9867\\
 & Transformer & 0.6571 & 0.9875 & 0.6514 & 0.9874\\
\hline
 & shallow & 0.1229 & 0.7922 & 0.1235 & 0.7910 \\
eICU & deep & 0.1550 & 0.8614 & 0.1567 & 0.8626\\
 & Transformer & 0.2499 & 0.9397 & 0.2515 & 0.9408\\
\hline
\end{tabular}
}
\end{table}

==> tables/structure_eval.tex <==
\begin{table}[t]
\vspace{-2mm}
\caption{KL divergence between the normalized true adjacency matrix and the attention map. We also show the entropy of the attention map to indicate the sparseness of the attention distribution. Parentheses denote standard deviations.}
\vspace{1mm}
\label{table:structure_eval}
\footnotesize
\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{lcccccc}
% \hline
\toprule
%Dataset & Model & \begin{tabular}{@{}c@{}} Validation\\Accuracy\end{tabular} & \begin{tabular}{@{}c@{}} Test\\Accuracy\end{tabular}\\

& \multicolumn{2}{c}{\textbf{Graph Reconstruction}} & \multicolumn{2}{c}{\textbf{Diagnosis-Treatment Classification}} & \multicolumn{2}{c}{\textbf{Masked Diagnosis Code Prediction}}\\
%\hline
%Model & \begin{tabular}{@{}c@{}} Validation\\Accuracy\end{tabular} & \begin{tabular}{@{}c@{}} Test\\Accuracy\end{tabular} & \begin{tabular}{@{}c@{}} Validation\\Accuracy\end{tabular} & \begin{tabular}{@{}c@{}} Test\\Accuracy\end{tabular}\\
Model & KL Divergence & Entropy & KL Divergence & Entropy & KL Divergence & Entropy\\
% \hline
\midrule
GCN$_P$ & 8.2250 & 1.8761 & 8.2250 & 1.8761 & 8.2250 & 1.8761\\
Transformer & 28.8123 & 1.6120 & 13.994 & 2.0953 & 15.1882 & 2.0230 \\
\mname & 7.6487 & 1.8788 & 8.5952 & 2.3143 & 9.0101 & 1.2618 \\
% \hline
\bottomrule
 %& GCN & 0.2828 & 0.3024\\
 %f& GCN$_P$ & 0.1908 & 0.2096\\
 %f& shallow & 0.3488 & 0.3417\\
%feICU & deep & 0.3549 & 0.3547\\
 %f& Transformer & 0.3647 & 0.3581\\
 %f& \mname & 0.2182 & 0.2328\\
%f\hline
\end{tabular}
%\vspace{-3mm}
}
\end{table}
